Deep learning of fMRI big data: a novel approach to subject-transfer decoding

As a technology to read brain states from measurable brain activities, brain decoding are widely applied in industries and medical sciences. In spite of high demands in these applications for a universal decoder that can be applied to all individuals simultaneously, large variation in brain activities across individuals has limited the scope of many studies to the development of individual-specific decoders. In this study, we used deep neural network (DNN), a nonlinear hierarchical model, to construct a subject-transfer decoder. Our decoder is the first successful DNN-based subject-transfer decoder. When applied to a large-scale functional magnetic resonance imaging (fMRI) database, our DNN-based decoder achieved higher decoding accuracy than other baseline methods, including support vector machine (SVM). In order to analyze the knowledge acquired by this decoder, we applied principal sensitivity analysis (PSA) to the decoder and visualized the discriminative features that are common to all subjects in the dataset. Our PSA successfully visualized the subject-independent features contributing to the subject-transferability of the trained decoder.

==> figures/fig0/caption.tex <==
\label{fig:cross_validation}
Cross validation

==> figures/fig0/size.tex <==
width=900

==> figures/fig1/caption.tex <==
How to train the neural networks.

==> figures/fig1/size.tex <==
width=800

==> figures/fig3/caption.tex <==
\label{fig:change_n}
Mean decoding accuracy plotted against the number of training subjects ($M$) in log scale.
Error bars indicate s.d. across ten cross validation iterations.

==> figures/fig3/size.tex <==
width=700

==> figures/fig_dnn/caption.tex <==
\label{fig:dnn}
We trained DNNs with the input being the fMRI scans and the output being their labeled task classes.

==> figures/fig_dnn/size.tex <==
width=700

==> figures/fig_prep/caption.tex <==
\label{fig:prep}
Preprocessing for each session data. 
For each session data, we applied voxel-wise z-score transformation, followed by averaging over each aROI. 
As a result, the dimension per fMRI scan was reduced to $116$.

==> figures/fig_prep/size.tex <==
width=400

==> figures/psa_final/caption.tex <==
\label{fig:PSA}
(a)
We calculated the first, second and third PSMs for each class. The PSMs of Motor and Social classes are shown here (see Appendix B Fig.\,\ref{fig:appendix_psa} for the other classes).
%
We recall that we intentionally omitted the class index in the formulation \eqref{eq:psm_rewrite} for simplicity, 
and that PSMs are actually meant to be computed for each class separately. 
% 
In the visualization of each PSM, we exclusivly colored the ROIs with values that are at least one s.d. away from the mean. 
%
Red and blue indicate different signs in the PSM values, i.e., the corresponding aROIs act oppositely in characterizing the class.
(b)
Similarity between maps was evaluated by cosine similarity.
We calculated the absolute value of cosine similarity (for definition, see the text) between all pairs of the first, second and third PSMs of the seven classes. Based on these similarity values, we applied a hierarchical clustering to the set of all the computed PSMs. 
The similarity matrix above is based on leaf order in the dendrogram (attached to the left side of the matrix) obtained by the hierarchical clustering. Intensity of the color indicates the degree of similarity.


==> figures/psa_final/size.tex <==
width=550
